Learning Embeddings for Image Clustering: An Empirical Study of Triplet Loss Approaches

In this work, we evaluate two different image clustering objectives, k-means clustering and correlation clustering, in the context of Triplet Loss induced feature space embeddings. Specifically, we train a convolutional neural network to learn discriminative features by optimizing two popular versions of the Triplet Loss in order to study their clustering properties under the assumption of noisy labels. Additionally, we propose a new, simple Triplet Loss formulation, which shows desirable properties with respect to formal clustering objectives and outperforms the existing methods. We evaluate all three Triplet loss formulations for K-means and correlation clustering on the CIFAR-10 image classification dataset.

==> 4_1_result_1_old.tex <==

\begin{figure}[t]
	\begin{center}
		%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
		\includegraphics[width=1.0\linewidth]{Fig_cifar10.pdf}
	\end{center}
	\caption{Margin $\alpha$ vs. Cluster Accuracy. Shown is the  accuracy for a wide range of margin parameter $\alpha$. The number in the bracket correspond to the equation number (e.g. regular Triplet Loss~\eqref{eq:triplet} is represented in gray). The addtional parameter $\beta$ for equation~\eqref{eq:triplet_add} and \eqref{eq:triplet_improved} set to $\beta=\alpha/2$.}
	\label{fig:cifar10}
\end{figure}

\subsection{Evaluation of Cluster Accuracy}
\label{subsec:result_acc}

Here, we investigate the clustering performance of the graph-based approach based on different loss functions when choosing a different $\alpha$.
We set the parameter for our Triplet Loss to $\beta=\alpha/2$.
The triplets are sampled randomly using the labels from the training dataset on CIFAR10. 
All experiments are executed five times with different random seeds and we report the average number and the standard deviation over the clustering accuracy.
\\

\textbf{Results.} 
Figure~\ref{fig:cifar10} shows the clustering accuracy for different margin parameter $\alpha$ on CIFAR10 test dataset. 
The clusters are obtained using multicut clustering.
First, we observe that increasing the margin parameter $\alpha$, the clustering accuracy consistently achieve higher performance across all three losses.
Furthermore, the regular Triplet Loss~\eqref{eq:triplet} (in gray) performs worse than the other two losses.
The highest performance is achieved when we train the CNN-model with the Triplet Loss~\eqref{eq:triplet_improved}, where the average accuracy is 80.2\%.
